Is Explanation the Cure? Misinformation Mitigation in the Short Term and Long Term

With advancements in natural language processing (NLP) models, automatic explanation generation has been proposed to mitigate misinformation on social media platforms in addition to adding warning labels to identified fake news. While many researchers have focused on generating good explanations, how these explanations can really help humans combat fake news is under-explored. In this study, we compare the effectiveness of a warning label and the state-of-the-art counterfactual explanations generated by GPT-4 in debunking misinformation. In a two-wave, online human-subject study, participants (N = 215) were randomly assigned to a control group in which false contents are shown without any intervention, a warning tag group in which the false claims were labeled, or an explanation group in which the false contents were accompanied by GPT-4 generated explanations. Our results show that both interventions significantly decrease participants' self-reported belief in fake claims in an equivalent manner for the short-term and long-term. We discuss the implications of our findings and directions for future NLP-based misinformation debunking strategies.

==> limitations.tex <==
\section*{Limitations}
In this survey, we adopted a warning-based method and an explanation-based
method. For the warning-based method, one limitation in this study was that
there are various types of warning labels: thus our results might not 
represent all types of warning labels. For instance, results might differ when using
``Disputed'' vs.\ ``This is fake news''.

For the explanation-based method, we sampled explanations that do not
contain model errors. The generation model might have errors and thus generate low-quality
fact-checked explanations. In our case, we only sampled explanations from 
those that had been examined as having no system error. Therefore, our
study does not count system errors.

Finally, in a real-world setting, the news detector could be wrongly classified as
fake news; we did not consider this possibility in this study. We verified the news claims in this survey. In a real-world environment, if the news were to detect true news as fake news, the warning label and explanation could have a negative influence.


\section*{Ethics Statement}

Our study has been approved by the Institutional Review Board of the authors’ institution.
We asked for informed consent from each participant.
We acknowledge that participants would inherently expose to the risk of reading fake news.
However, prior studies showed that misinformation studies did not significantly increase participants’ long-term susceptibility to misinformation used in the experiments~\cite{murphy2020fool}. 
We also informed participants that they have the right to leave the experiment whenever they want.



\section*{Acknowledgements}

